On Benchmarking Embedded Linux Flash File Systems

Due to its attractive characteristics in terms of performance, weight and power consumption, NAND flash memory became the main non volatile memory (NVM) in embedded systems. Those NVMs also present some specific characteristics/constraints: good but asymmetric I/O performance, limited lifetime, write/erase granularity asymmetry, etc. Those peculiarities are either managed in hardware for flash disks (SSDs, SD cards, USB sticks, etc.) or in software for raw embedded flash chips. When managed in software, flash algorithms and structures are implemented in a specific flash file system (FFS). In this paper, we present a performance study of the most widely used FFSs in embedded Linux: JFFS2, UBIFS,and YAFFS. We show some very particular behaviors and large performance disparities for tested FFS operations such as mounting, copying, and searching file trees, compression, etc.

==> 1_FlashMemoryManagement.tex <==
\section{Flash memory management\\with Linux}

One can identify two ways for flash-based devices management under Linux :
\begin{itemize}
  \item The use of the \textit{Flash Translation Layer} \cite{gal_algorithms_2005, gupta_dftl_2009}, an hardware layer located inside the controller of flash-based devices such as USB flash drives, SD/MMC cards, and SSDs. The FTL emulates a block device allowing the peripheral to be formated with a standard file system, and performs a logical to physical address mapping through which is done the \textit{wear leveling} ;
  \item The use of dedicated \textit{Flash File Systems} (FFSs) \cite{egger_file_????, guido_r._kok_flash_2008, woodhouse_jffs:_2001, adrian_hunter_brief_2008, adrianhunter_ubifs_????, wookey_yaffs_2007, manning_how_2010}, commonly used in embedded-board based devices with raw flash chips, such as smartphones, set top boxes, and a large set of embedded systems. 
\end{itemize}

In the case of FFS, the file system is in charge of garbage collection and wear leveling operations, in addition to the standard file management operation.

